A Note on the Expressiveness of BIP

We extend our previous algebraic formalisation of the notion of component-based framework in order to formally define two forms, strong and weak, of the notion of full expressiveness. Our earlier result shows that the BIP (Behaviour-Interaction-Priority) framework does not possess the strong full expressiveness. In this paper, we show that BIP has the weak form of this notion and provide results detailing weak and strong full expressiveness for classical BIP and several modifications, obtained by relaxing the constraints imposed on priority models.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{D. Gebler and K. Peters (Eds.): Combined Workshop on Expressiveness in\\
Concurrency and Structural Operational Semantics (EXPRESS/SOS 2016).\\
EPTCS 222, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.222.1}{10.4204/EPTCS.222.1}}
\pdfoutput=1

